Controlling the propagation of light in disordered scattering media

This thesis describes experimental work on the use of wavefront shaping to steer light through strongly scattering materials. We find that scattering does not irreversibly scramble the incident wave. By shaping the incident wavefront, we make opaque objects focus light as sharply as aberration free lenses. We use feedback from a target behind, or in, an opaque object to shape the incident wave. This way, light is focused through, or inside, opaque objects for the first time ever.

==> sectiontitles.tex <==
%redefine chapter title layout
%----------------------------------------------------------
\makeatletter %(required to be able to use internal LaTeX macros, ended by \makeatother)
\def\@makechapterhead#1{%
  {\raggedright \sffamily
    \interlinepenalty\@M
    \huge Chapter \thechapter\\
    \linespread{0.95}
    \Huge \bfseries #1\par\nobreak
    \vskip 40\p@
  }}
\def\@makeschapterhead#1{%(for chapter*)
  {\raggedright \sffamily
    \interlinepenalty\@M
    \linespread{0.95}
    \Huge \bfseries #1\par\nobreak
    \vskip 40\p@
  }}

%redefine layout for section, subsection and subsubsection titles
%----------------------------------------------------------------
\renewcommand\section{\@startsection{section}{1}{\z@}%
  {-3.5ex \@plus -1ex \@minus -.2ex}% spacing before title
  {1.3ex \@plus.15ex}% spacing after title
  {\raggedsection\normalfont\sectfont\nobreak\size@section}% title line font(\sectfount = sans serif)
}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
  {-3.25ex\@plus -1ex \@minus -.2ex}%
  {0.8ex \@plus .1ex}%
  {\raggedsection\normalfont\sectfont\nobreak\size@subsection}%
}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
  {-3.25ex\@plus -1ex \@minus -.2ex}%
  {0.8ex \@plus .1ex}%
  {\raggedsection\normalfont\sectfont\nobreak\size@subsubsection}%
}

\makeatother

